HPE:Answering Complex Questions over Text by Hybrid Question Parsing and Execution

The dominant paradigm of textual question answering systems is based on end-to-end neural networks, which excels at answering natural language questions but falls short on complex ones. This stands in contrast to the broad adaptation of semantic parsing approaches over structured data sources (e.g., relational database, knowledge graphs), that convert natural language questions to logical forms and execute them with query engines. Towards combining the strengths of neural and symbolic methods, we propose a framework of question parsing and execution on textual QA. It comprises two central pillars: (1) We parse the question of varying complexity into an intermediate representation, named H-expression, which is composed of simple questions as the primitives and symbolic operations representing the relationships among them; (2) To execute the resulting H-expressions, we design a hybrid executor, which integrates the deterministic rules to translate the symbolic operations with a drop-in neural reader network to answer each decomposed simple question. Hence, the proposed framework can be viewed as a top-down question parsing followed by a bottom-up answer backtracking. The resulting H-expressions closely guide the execution process, offering higher precision besides better interpretability while still preserving the advantages of the neural readers for resolving its primitive elements. Our extensive experiments on MuSiQue, 2WikiQA, HotpotQA, and NQ show that the proposed parsing and hybrid execution framework outperforms existing approaches in supervised, few-shot, and zero-shot settings, while also effectively exposing its underlying reasoning process.

==> Table/lf_3example.tex <==
\begin{table*}[]
\centering
\renewcommand{\arraystretch}{0.9}
\resizebox{\textwidth}{!}{
\begin{tabular}{ll}
\toprule
\multirow{2}{*}{\textbf{Bridge}}       & \textit{Question: Where was the place of film The Iron Man director?}                                                                      \\ 
                              & JOIN ( QA( \underline{Where is Ans\#1's place of death?} ), QA( \underline{Who is director of The Iron Man?} ) )                                             \\ 
                                & ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~Question\#2   ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~ Question\#1 \\ \hline
\multirow{2}{*}{\textbf{Intersection}} & \textit{Question: Which team is Bernard Lowe was a member of beat the winner of the 1894-95 FA Cup?}                                       \\ 
                              & AND ( QA( \underline{What is member of sports team of Bernard Lowe?} ) , QA( \underline{Who won the 1894-95 FA Cup?} ) )                                 \\ 
                                & ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~Question\#2   ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~ Question\#1 \\ \hline
\multirow{2}{*}{\textbf{Comparison}}   & \textit{Question: Did Lenny Mchallister and Ken Xie have the same nationality?}                                                             \\ 
                              & COMPARE\_= ( QA( \underline{What is the nationality of Lenny Mchallister?} ), QA( \underline{What is the nationality of Ken Xie?} ) )\\ 
                                & ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~Question\#2   ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~ Question\#1 \\ 
\bottomrule
\vspace{-1.5em}
\end{tabular}
}
\caption{Examples of question and corresponding H-expression under three basic reasoning types. For more complex reasoning types, their questions and H-expressions are shown in the Appendix \ref{sec:musique}. }
\label{tb_lfexample}
\end{table*}

==> Table/lf_example.tex <==
\begin{table}[]
\begin{tabular}{llll}
Reasoning Type & Question   & Decomposition   & Logical Form                                                                                                                                                          \\
2hop1entity    & \begin{tabular}[c]{@{}l@{}}Who succeeded the first \\ President of Namibia?\end{tabular}                                                                     & \begin{tabular}[c]{@{}l@{}}1. Who was the first President of Namibia? Ans: \#1\\ 2. Who succeeded \#1?\end{tabular}                                                                & \begin{tabular}[c]{@{}l@{}}JOIN(Who succeeded \#1, \\ Who was the first President of Namibia?)\end{tabular}                                                           \\
1hop2entity    & \begin{tabular}[c]{@{}l@{}}When was the first establishment that \\ McDonaldization is named after, open \\ in the country Horndean is Located?\end{tabular} & \begin{tabular}[c]{@{}l@{}}1. What is McDonaldization named after? Ans: \#1\\ 2. Which state is Horndean located in? Ans:\#2\\ 3. When did the first \#1 open in \#2?\end{tabular} & \begin{tabular}[c]{@{}l@{}}JOIN(When did the first \#1 open in \#2,\\ AND(What is McDonaldization named after, \\ Which state is Horndean located in? ))\end{tabular}
\end{tabular}
\label{lf_example}
\end{table}

==> Table/table_texpression.tex <==
\begin{table}[h]
\setlength{\tabcolsep}{3pt}
\centering
\resizebox{1\linewidth}{!}{
\begin{tabular}{lll}
\toprule 
\textbf{Operation}      & \textbf{Return}       & \textbf{Description}  \\ \midrule
{\sc{join}} [q2(a1), q1] & Text span & \begin{tabular}[c]{@{}l@{}} q2's execution depends on q1's answer \\ to replace the placeholder a1. \\ Finally returns q2's answer.\end{tabular}    \\ \midrule
{\sc{union}} [q2, q1] & Text spans  & Returns q2 and q1's answers as a list.                  \\ \midrule
{\sc{intersect}} [q2, q1] & Text spans  & Returns intersection of q2 and q1's answers.                  \\ \midrule
{\sc{comp}}\_= [q2, q1] & Yes/No  & \begin{tabular}[c]{@{}l@{}}Compare if the answers of q2 and q1 are equal. \end{tabular}  \\ \midrule
\begin{tabular}[c]{@{}l@{}}{\sc{comp}}\_\textgreater{} [q2, q1] \\ {\sc{comp}}\_\textless{} [q2, q1]\end{tabular} & \begin{tabular}[c]{@{}l@{}}Main Entity\\ in q2/q1\end{tabular} & \begin{tabular}[c]{@{}l@{}}Compare the answers of q2 and q1 \\ and return the main entity of q2 or q1.\end{tabular} \\ \midrule
{\sc{sub}} [q2, q1]    & Number    & \begin{tabular}[c]{@{}l@{}} Subtract q1's numeric answer from q2's answer. \end{tabular}   \\ \midrule
{\sc{add}} [q2, q1]    & Number  & \begin{tabular}[c]{@{}l@{}} Add q2's and q1's numeric answers. \end{tabular}   \\
\bottomrule                                                                      \end{tabular}
}
\caption{Operations defined in our H-expressions; q2 and q1 are single-hop natural questions.}
\label{table_texpression}
\end{table}
